Asynchronous Federated Optimization

Federated learning enables training on a massive number of edge devices. To improve flexibility and scalability, we propose a new asynchronous federated optimization algorithm. We prove that the proposed approach has near-linear convergence to a global optimum, for both strongly convex and a restricted family of non-convex problems. Empirical results show that the proposed algorithm converges quickly and tolerates staleness in various applications.

==> related_work.tex <==
\section{Related work}

Edge computing~\cite{garcia2015edge,hong2013mobile} is increasingly employed in various scenarios such as smart homes, wearable devices, and sensor networks. At the same time, machine-learning applications are increasingly moving from the cloud to the edge~\cite{cao2015distributed,mahdavinejad2018machine,zeydan2016big}. Typically, edge devices have weaker computation and communication capacity compared to workstations and data centers, due to the weaker hardware, limited battery, and metered networks. As a result, simple machine-learning models such as MobileNet~\cite{howard2017mobilenets} have been proposed for learning with weak devices.

Existing federated optimization methods~\cite{konevcny2015federated,konevcny2016federated,mcmahan2016communication,bonawitz2019towards} focus on synchronous training. In each global epoch, the server triggers training tasks on a subset of workers. However, perhaps due to bad networking conditions and occasional issues, some worker may fail. When this happens, the server has to wait until a sufficient number of workers respond — otherwise, the server times out,  drops the current epoch, and moves on to the next epoch. As far as we know, this paper is the first to consider asynchronous training in federated learning theoretically and empirically.

Asynchronous training~\cite{zinkevich2009slow,lian2017asynchronous,zheng2017asynchronous} is widely used in traditional distributed stochastic gradient descent (SGD). While comparing synchronous and asynchronous SGD can be nuanced and depend on system details, previous work often observes that asynchronous SGD can converge faster than synchronous SGD, particularly when the communication latency is high and heterogeneous~\cite{zinkevich2009slow,lian2017asynchronous,zheng2017asynchronous}. While classic asynchronous SGD requires directly sending gradients from the workers to the server after each local update, such an approach is not feasible for edge devices due to unreliable and slow communication -- hence the prevalence of standard federated averaging that send model parameters after several local updates~\cite{konevcny2015federated,konevcny2016federated,mcmahan2016communication,bonawitz2019towards}. Taken together, our approach takes advantage of asynchronous training and combines it with federated optimization.
